Streamlining Cloud-Native Application Development and Deployment with Robust Encapsulation

Current Serverless abstractions (e.g., FaaS) poorly support non-functional requirements (e.g., QoS and constraints), are provider-dependent, and are incompatible with other cloud abstractions (e.g., databases). As a result, application developers have to undergo numerous rounds of development and manual deployment refinements to finally achieve their desired quality and efficiency. In this paper, we present Object-as-a-Service (OaaS) -- a novel serverless paradigm that borrows the object-oriented programming concepts to encapsulate business logic, data, and non-functional requirements into a single deployment package, thereby streamlining provider-agnostic cloud-native application development. We also propose a declarative interface for the non-functional requirements of applications that relieves developers from daunting refinements to meet their desired QoS and deployment constraint targets. We realized the OaaS paradigm through a platform called Oparaca and evaluated it against various real-world applications and scenarios. The evaluation results demonstrate that Oparaca can enhance application performance by 60X and improve reliability by 50X through latency, throughput, and availability enforcement -- all with remarkably less development and deployment time and effort.

==> abstract.tex <==
\begin{abstract}

% Cloud computing has become a de facto paradigm for modern services, reshaping the way businesses and individuals construct, deploy, and deliver their solutions.
% Cloud services are typically offered through high-level abstractions that hide the infrastructure complexity to simplify and accelerate software production cycles.
Cloud services rely on high-level abstractions to hide infrastructure complexity, simplifying and accelerating software production cycles.
% However, most of the current Cloud abstractions poorly support non-functional requirements (i.e., QoS and constraints) and are incompatible across cloud providers.
However, current abstractions often lack support for non-functional requirements (e.g., QoS and constraints) and are incompatible across providers.
As a result, application developers still have to undergo numerous rounds of development and manual deployment refinements to achieve their desired quality and efficiency.
% limited non-functional requirement supports so cloud-native applications still have to manage their quality manually that may end up with low productivity, poor resource use, complicated and costly performance control.
In this paper, we present Object-as-a-Service (OaaS)---a serverless paradigm that borrows the object-oriented programming concepts to encapsulate application logic, data, and non-functional requirements
into a single deployment package, thereby streamlining provider-agnostic cloud-native application development. We also propose a declarative interface for the non-functional requirements of applications that relieves developers from daunting refinements to meet their desired QoS and deployment constraint targets. We realized the OaaS paradigm through a platform called Oparaca and evaluated it against various real-world applications and scenarios.
% The evaluation results show that Oparaca can achieve a comparable efficiency with other state-of-the-art approaches, while remarkably reducing the time and effort of cloud-native application development and deployment. 
The evaluation results show that via latency, throughput, and availability enforcement, Oparaca can improve application performance by 60x and 50x more reliability with remarkably less development and deployment time and effort.

\end{abstract}

% \begin{IEEEkeywords}
% Cloud computing, Cloud-native application development, FaaS, Serverless paradigm, Object-as-a-Service (OaaS) abstraction, Quality of Service
% \end{IEEEkeywords}

==> implementation.tex <==
\section{Implementation (1 page)}
\label{sec:implementation}

% \textbf{Considering merge this with Architecture}

In this section, we will present how components mentioned in the OaaS Architecture are implemented and combined to with each other to deploy and maintain an OaaS package over the cloud.

% \subsection{Dynamic Class Runtime Concept}

% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{Figures/qos_oaas_high_level.dio.pdf}
%     \caption{High-level architecture (temporary) NOTE: ideally, it should highlight dynamical class runtime.}
%     \label{fig:class-runtime}
% \end{figure}

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{Figures/qcoaas_flow.dio.pdf}
    \caption{Flow of Class runtime realization (need to simplify and change orbit to CR)}
    \label{fig:runtime-realization}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=1\linewidth]{Figures/qos_oaas_architecture_v15_2.dio.pdf}
    \caption{Class Runtime Implementation}
    \label{fig:enter-label}
\end{figure}


% Figure \ref{fig:class-runtime} shows how the objects defined by the interface will be deployed and managed over the cloud through class runtime. 
% Particularly, the class runtime is a set of components that execute the class logic provided by developers. In order to meet the third requirement, the class runtime must be flexible enough to fulfill the non-functional requirements of different classes. It is impractical to have a single design for the class runtime that can satisfy all of the requirements. It also eliminates the possibility of providing specialized runtime for specific use cases. Therefore, the class runtime must be dynamic, extendable, and dedicated to a specific combination of non-functional requirements. This way, each class runtime can be optimized and scaled independently. To simplify matters, each class runtime should be dedicated to a single class.  

% To make the class runtime extendable, we introduce the concept of a \textit{class runtime template}. The platform provider can extend new runtime by adding the new template.  

% template parameters:
% \begin{itemize}
%     \item default system parameters (e.g., requested CPU and memory)
%     \item implementation and configuration of optimizer 
%     \item implementation and configuration of components within class runtime
%     \item condition (e.g., matched QoS or constraints) and priority to select this template
% \end{itemize}

% In order to deploy the new class runtime for the newly registered class definition, the platform will search through the list of templates and select the one with the highest priority and meet the condition. Then the system can realize the  
%  deployment configuration of this class runtime by running the associated optimizer.  Before deploying, the configuration is used for estimating the amount of resources needed and validating if it is feasible to deploy with the given current cluster environment. If it fails, the fallback mechanism will be applied and reported back to developers. Otherwise, the system can process the deployment by translating it into the deployment configuration and submitting it to the orchestrator.

\subsection{Automated Optimization of Class Runtime}

In order to effectively meet the non-functional requirement, the class runtime has to be automatically adjusted/optimized when the environment or workload changes. The steps of automatically adjusting/optimizing are shown in Figure \ref{fig:runtime-realization}. Overall, these steps can be groups into four phases
\begin{itemize}
    \item \textit{Monitoring}: The class runtime continuously exports its metrics to the monitoring system. \textbf{TODO: Highlight parts of the figure used in the phase + explanation}
    \item \textit{Change Detection}: The platform periodically aggregates the metrics to detect if the configuration has to be regenerated because of the workload/environment change. \textbf{TODO: Highlight parts of the figure used in the phase + explanation}
    \item \textit{Configuration Evaluation}: Re-validating the feasibility of class runtime if it can meet the non-functional requirement. \textbf{TODO: Highlight parts of the figure used in the phase + explanation}
    \item \textit{Reconfiguration} re-apply the configuration if it is needed. \textbf{TODO: Highlight parts of the figure used in the phase + explanation}
\end{itemize}

To explain more deeper about the whole process, let us show how Oparaca enforces object throughput and availability under a restricted budget constraint as representative examples.

\subsubsection{Throughput Enforcement}
\textbf{TODO: describe algorithm to guarantee throughput}
\vspace{1in}

\subsubsection{Availability Enforcement}
\textbf{TODO: describe algorithm to guarantee availability}

\color{blue}
$failure\_probability = (1 - infra\_avail)^{replicas}$

$1 - target\_avail = (1 - infra\_avail)^{replicas}$

$log(1 - target\_avail) = replicas \cdot log(1 - infra\_avail)$

$replicas = \frac{log(1-target\_avail)}{log(1-infra\_avail)}$

$min\_replicas = max(ceil(\frac{log(1-target\_avail)}{log(1-infra\_avail)}), 1)$

\color{black}
\vspace{1in}

\subsubsection{Satisfying Budget Constraint}
\textbf{TODO: describe how to budget constraint act will be enforced, consider removing this if we already cover it in the other subsections}
\vspace{1in}


% \subsection{Object Invocation (function call)}
% Interaction between modules:
% \begin{itemize}
%     \item LB (for single endpoint)
%     \item Object Module (invoker, distributed in-memory hash table with consistent hashing, and invocation offloading)
%     \item FaaS engine (presigned URL)  
%     \item Persistent data Module 
%     \item metrics collecting (invocation timer)
% \end{itemize}

% \subsection{Class Registration}
% \textcolor{red}{NOT SURE IF STILL NEEDED (MERGE TO DYNAMIC CLASS RUNTIME)}
% \begin{itemize}
%     \item Class submission to Package Manager
%     \item Forward the definitions into the corresponding class runtime manager 
%     \item Class runtime template selection
%     \item Class runtime realization 
%     \item Static Feasibility Check
% \end{itemize}



% \subsection{Automated Optimization}
% \textcolor{red}{DUPLICATED WITH PREVIOUS SECTION}
% \begin{itemize} %Loop 
%     \item  Monitoring 
%     \item  Class Runtime Manager
%     \item  Finding the optimized configuration
%     \item  Runtime Feasibility Check
% \end{itemize}


==> oaas-backgound.tex <==
\subsection{State Management Strategies}
The idea of stateful serverless is explored in several research works. 
As noted in Figure~\ref{fig:stateful_serverless} and Table~\ref{tab:ssls-comp}, these works can be categorized into \emph{actor model}, \emph{datastore abstraction}, and \emph{pure function} approaches depending on where the platform stores the state data, and how the function accesses the data. According to Figure \ref{fig:stateful_serverless}, the actor model places the state inside the worker node (instance) to achieve the data locality. In the pure function, however, the state is placed on other systems (\eg database) and is transferred to the worker instance upon invocation. Hence, the state appears as part of the function input argument, and the modified state appears as its output. Thus, the function is still stateless while exhibiting stateful features. The datastore abstraction is a hybrid approach where the platform provides the API for the function to access the data on demand. Depending on the design, the state might be stored in the database but can also be cached in the worker.

\begin{figure}[tbp]
  \centering
  \includegraphics[width=0.48\textwidth]{Figures/stateful_serverless.pdf}
  \caption{\small{The illustrated comparison of three different models of stateful serverless.}}
  \vspace{-2mm}
  \label{fig:stateful_serverless}
\end{figure}

\begin{table}[tbp]
\begin{tabular}{c|c|c|c}
                                                                          & \small{\textbf{\begin{tabular}[c]{@{}c@{}}Actor \\ Model\end{tabular}}}                         & \small{\textbf{\begin{tabular}[c]{@{}c@{}}Datastore\\ Abstraction\end{tabular}}}                   & \small{\textbf{\begin{tabular}[c]{@{}c@{}}Pure\\  Function\end{tabular}}}             \\ \hline \hline
\small{\textbf{\begin{tabular}[c]{@{}c@{}}\small{Data} \\ \small{placement}\end{tabular}}}        & \small{\begin{tabular}[c]{@{}c@{}}worker \\ instances\end{tabular}}                             & \small{\begin{tabular}[c]{@{}c@{}}platform services\\ or database\\ (depend on impl.)\end{tabular}} & \small{\begin{tabular}[c]{@{}c@{}}platform \\ services\\ or database\end{tabular}} \\ \hline
\small{\textbf{Complexity}}                                                       & \small{high}                                                                                    & \small{depend on impl.}                         & \small{low}                                                                           \\ \hline
\small{\textbf{Data locality}}                                                    & \small{high}                                                                                    & \small{depend on impl.}                         & \small{low}                                                                           \\ \hline
\small{\textbf{\begin{tabular}[c]{@{}c@{}}Unstructured \\ data support\end{tabular}}}     & \small{difficult}                             & \small{yes}                                                                                   & \small{difficult}                                                                     \\ \hline
\small{\textbf{\begin{tabular}[c]{@{}c@{}}Deployment\\ granularity\end{tabular}}} & \small{\begin{tabular}[c]{@{}c@{}}actor\\ (multiple\\functions)\end{tabular}}                   & \small{function}                                                                                    & \small{function}                                                                      \\ \hline
\small{\textbf{\begin{tabular}[c]{@{}c@{}}Maintain-\\ ability\end{tabular}}}                                                  & \small{low}                                                                                     & \small{high}                                                                                        & \small{high}                                                                          \\ \hline
\small{\textbf{Solutions}}                                                        & \small{\begin{tabular}[c]{@{}c@{}}Kalix~\cite{kalix},\\ Azure Entity \\ Func.\cite{azure_enfunc},\\
Cepless~\cite{cepless}
\end{tabular}} & \small{\begin{tabular}[c]{@{}c@{}}
Cloudburst~\cite{cloudburst},\\
FAASM~\cite{faasm},\\ 
Apiary~\cite{kraft2022apiary},\\
Crucial~\cite{crucial},\\
Boki~\cite{jia2021boki},\\
Beldi~\cite{beldi},\\
\textbf{\sysname}\end{tabular}}                                 & \small{\begin{tabular}[c]{@{}c@{}}Kalix~\cite{kalix}\\
% eigr~\cite{eigr},\\ 
Statefun~\cite{statefun}, \\
\textbf{\sysname}\end{tabular}}   
\end{tabular}
\caption{\label{tab:ssls-comp}\small{Comparing properties of various design patterns to build a stateful serverless platform.}}
\vspace{-4mm}
\end{table}


According to Table~\ref{tab:ssls-comp}, the actor model serverless platform needs to maintain the availability of each actor (object) where both data and compute reside. Maintainability is particularly difficult for bulky unstructured data because the platform needs to balance the computing and storage aspects of each node. In addition, the platform has to support a routing mechanism to navigate a function call to the actor's location. Alternatively, the pure function approach disaggregates the state management and compute (function) for the sake of system design simplicity. However, it compromises the data locality aspect. Similar to pure functions, datastore abstraction also relaxes the need to store the state on the worker node. Regardless, it utilizes caching techniques to preserve data locality. The deployment granularity of the actor model approach is an actor with multiple functions that share the same state, whereas the granularity in other approaches is a single function. 

The actor model approach has been popular in programming languages and OOP, because it spurs asynchronous messaging across actors and lends itself to distributed deployments. That is why it has been an attractive choice for stateful serverless platforms, even though it poorly supports unstructured data. Kalix~\cite{kalix} and Azure Entity Functions~\cite{azure_enfunc}, which are part of Azure durable functions, are example platforms implemented based on the actor model approach. The serverless platforms based on the datastore abstraction are mostly popular in research. Cloudburst~\cite{cloudburst} offers stateful functions using a shared distributed key-value database to keep track of the state. FAASM~\cite{faasm} optimizes the function-state interaction overhead via employing web assembly \cite{wasm}. Even though web assembly enables multiple functions to share the memory and achieve data locality, it implies compiling the code into web assembly, which limits the compatibility of some libraries.
Crucial~\cite{crucial} allows a function to access the shared data via the DSO layer (distributed hash table).
Boki~\cite{jia2021boki} enables stateful function via providing API access to the distributed logging system. Beldi~\cite{beldi}, on the other hand, provides the database and transaction API to the state.
Apache Flink Stateful Function (StateFun) \cite{statefun}, 
and Kalix~\cite{kalix} are solutions based on the pure function approach. Statefun is built atop Apache Flink based on the actor model. However, it offloads the function code to a dedicated worker that can be categorized under the pure function approach. 

==> rts-impl.tex <==
Real-time Serverless Implementation (Pre-allocation Approach) -- only work effectively with constant-rate workloads.
The algorithm:
    Input:
        - rate, max execution time --> the deployment configurations (given constants, we dont need to infer them from monitoring)
    Algorithm:
        - Reserve X instances where
            X = rate * max execution time / concurrency
            X is the MINIMUM required instances to meet the guarantee, we have allocate more than X if needed.

How do we implement the alogrithm only through KNative function configurations?

What does KNative give us? 
- Resource per per instance.
    RequestMemory,
    RequestCPU,
    LimitCPU,
    LimitMemory
- Concurrency = number of invocation/instance.
- Timeout
- minInstances
- maxInstances

What will we do with these:
Set:
    - - concurrency = hard concurrency (10 invocation/instance)
    - Timeout = max execution time
    - minInstances = X
    - maxInstances = X + 1


How to find the maximum throughput?

    - Hai:
        - Continuously send 1 new invocation request for every T second.
        - varying input rate (by changing T)
        - start with small input rate (large T, probably start with 1s --> 1 request/sec), measure the throughput we should get the throughput == input rate, otherwise, try again with a bigger T.
            - Increase input rate (reduce T, for example 1 --> 0.9 --> 0.8 --> etc.) until throughput < input rate --> value of input rate where the throughput stop being equal to the input is the maximum throughput.

            Do binary search:
                - start with a very small one --> OK
                - start with a very large one --> Collapse
                - take average of the two, repeat


 0.1s: 10c => 100rps
    - Wis:
      generate req with concurrency rate of #c in [x:y]
      each increment will increase the throughput (completion rate) until it is stopped (or extremely slow down) at T, which is the maximum throughput
    

